Robust Multiview Multimodal Driver Monitoring System Using Masked Multi-Head Self-Attention

Driver Monitoring Systems (DMSs) are crucial for safe hand-over actions in Level-2+ self-driving vehicles. State-of-the-art DMSs leverage multiple sensors mounted at different locations to monitor the driver and the vehicle's interior scene and employ decision-level fusion to integrate these heterogenous data. However, this fusion method may not fully utilize the complementarity of different data sources and may overlook their relative importance. To address these limitations, we propose a novel multiview multimodal driver monitoring system based on feature-level fusion through multi-head self-attention (MHSA). We demonstrate its effectiveness by comparing it against four alternative fusion strategies (Sum, Conv, SE, and AFF). We also present a novel GPU-friendly supervised contrastive learning framework SuMoCo to learn better representations. Furthermore, We fine-grained the test split of the DAD dataset to enable the multi-class recognition of drivers' activities. Experiments on this enhanced database demonstrate that 1) the proposed MHSA-based fusion method (AUC-ROC: 97.0\%) outperforms all baselines and previous approaches, and 2) training MHSA with patch masking can improve its robustness against modality/view collapses. The code and annotations are publicly available.

==> 4-experiments/8-visualization.tex <==
\subsection{Result Visualization}



==> floats/tables/backbone.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
{\tabulinesep=0.3em
\begin{tabu}{l|l|l}
\hline
\textbf{Layer Name} & \textbf{Output Size}    & \textbf{Layer Structure}                                                                            \\ \hline
conv1               & $8 \times 56 \times 56$ & \begin{tabular}[c]{@{}l@{}}$3 \times 7 \times 7$, 64,\\ stride $1 \times 2 \times 2$\end{tabular}   \\ \hline
conv2               & $8 \times 56 \times 56$ & $\begin{bmatrix} 3 \times 3 \times 3, \, 64 \\ 3 \times 3 \times 3, \, 64 \end{bmatrix} \times 2$ \\ \hline
conv3               & $4 \times 28 \times 28$ & $\begin{bmatrix} 3 \times 3 \times 3, \, 128 \\ 3 \times 3 \times 3, \, 128 \end{bmatrix} \times 2$ \\ \hline
conv4               & $2 \times 14 \times 14$ & $\begin{bmatrix} 3 \times 3 \times 3, \, 256 \\ 3 \times 3 \times 3, \, 256 \end{bmatrix} \times 2$ \\ \hline
conv5               & $1 \times 7 \times 7$   & $\begin{bmatrix} 3 \times 3 \times 3, \, 512 \\ 3 \times 3 \times 3, \, 512 \end{bmatrix} \times 2$ \\ \hline
\end{tabu}%
}
}
\caption{The configuration of the R3D-18 backbone \cite{tran2018closer} (with the input size $8 \times 112 \times 112$). Those within the brackets are the kernel size $(t \times h \times w)$ and the output channels $c$ of each residual block. The number outside is the times that the residual block is repeated. }
\label{tbl:backbone}
\end{table}


==> floats/tables/multiple_acc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\definecolor{best}{HTML}{ff0054}

\begin{table}[tb]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|ccccc}
\hline
\textbf{Source}               & Sum & Conv & SE & AFF & MHSA                   \\ \hline
\textbf{Top (D)}          & \multicolumn{5}{c}{84.6}                  \\
\textbf{Top (IR)}         & \multicolumn{5}{c}{84.5}                  \\
\textbf{Top (D+IR)}     & 82.9 & 83.8 & 83.8 & 84.0 & \textbf{84.3} \\ \hline
\textbf{Front (D)}        & \multicolumn{5}{c}{83.3}                  \\
\textbf{Front (IR)}       & \multicolumn{5}{c}{83.0}                  \\
\textbf{Front (D+IR)}   & 83.8 & 85.3 & 85.4 & 85.4 & \textbf{86.1} \\ \hline
\textbf{Top+Front (D)}  & 87.3 & 87.7 & 87.5 & 87.8 & \textbf{87.9} \\
\textbf{Top+Front (IR)} & 87.9 & 87.8 & 87.9 & 88.0 & \textbf{88.2} \\
\textbf{Top+Front (D+IR)} & 88.1         & 88.2          & 88.2        & 88.2         & {\color{best} \textbf{88.4}} \\ \hline
\end{tabular}%
}
\caption{The accuracies (\%) of close-set multiclassification. For each data source, the highest score is \textbf{bolded}, and the overall best score is shown in \color{best}{red}. \TG{This table is redundant in my opinion. Should be removed.}}
\label{tbl:mutli_acc}
\end{table}

